Extended Version of GTGraffiti: Spray Painting Graffiti Art from Human Painting Motions with a Cable Driven Parallel Robot

We present GTGraffiti, a graffiti painting system from Georgia Tech that tackles challenges in art, hardware, and human-robot collaboration. The problem of painting graffiti in a human style is particularly challenging and requires a system-level approach because the robotics and art must be designed around each other. The robot must be highly dynamic over a large workspace while the artist must work within the robot's limitations. Our approach consists of three stages: artwork capture, robot hardware, and planning & control. We use motion capture to capture collaborator painting motions which are then composed and processed into a time-varying linear feedback controller for a cable-driven parallel robot (CDPR) to execute. In this work, we will describe the capturing process, the design and construction of a purpose-built CDPR, and the software for turning an artist's vision into control commands. Our work represents an important step towards faithfully recreating human graffiti artwork by demonstrating that we can reproduce artist motions up to 2m/s and 20m/s$^2$ within 9.3mm RMSE to paint artworks. Changes to the submitted manuscript are colored in blue.

==> __latexindent_temp.tex <==
{1}{2}w^{t}w+C\sum_{i=1}^{N}{\xi_{i}}}
  {}{}
  \addConstraint{y_{i}(w\phi(x_{i}+b))+\xi_{i}-1}
  \addConstraint{\xi\geq0}{}
  \end{mini*}

==> old_09-06/2_mechanical.tex <==
% Cable Driven Parallel Robots (CDPR) are ideally suited for the challenging task of painting graffiti art.
% % due to the large scale, the fast, fluid motion required, and the artistic components to obtaining and generating trajectories which demand limited constraints on motion planning.
% A graffiti painting robot operates on a large scale -- it should be able to cover the side of an entire building -- and it should also posses great speed and fluidity since, like many art forms, graffiti represents some of the most skilled maneuvers humans perform.  CDPRs possess both of these capabilities.  A CDPR is a robot whose end-effector is pulled by a (redundant) set of cables which are driven by winches on a fixed base.  Thanks to properties of cables, CDPRs can scale to extraordinary sizes and speeds \cite{Nan11ijmp_FAST_telescope, Saptarshi20nasa_lunartelescope}, with the limitation of reduced stiffness to external wrenches, making them ideally suited to the large but relatively undisturbed setting for graffiti painting.
% Furthermore, extensive studies in the late 2000's of CDPR workspace analysis \cite{Bosscher06TRO_wrenchFeasible, Bouchard09_WFW, Gouttefarde11TRO_cableWFW} make possible the hierarchical planning and control required for artistic components regarding composition of shapes, infill, and order of execution.


% The primary focus of CDPR research has been on workspace analysis, control, and estimation.  Wrench-closure and later wrench-feasible workspaces, which refer to the configurations that can produce desired wrenches on the end-effector given constraints of positive cable tensions and bounded cable tensions respectively, have been more-or-less solved numerically and can be computed offline based on the CDPR geometry \cite{Bosscher06TRO_wrenchFeasible, Bouchard09_WFW, Gouttefarde11TRO_cableWFW}.  For real-time control, a great deal of work has focused both on cable-suspended parallel robots (CSPR) and CDPR.  While CDPR are overactuated, CSPR are not which cause them to typically experience greater degrees of oscillation and cable sag complicating which require compensation \cite{Ida18_cableRestToRest, Tang13_cable_telescope}. % Tang13 is not a great reference here (gerry)
% Meanwhile, CDPR control places emphasis on redundancy resolution \cite{Miermeister16iros_CableRobotSimulator, Pott09ckin_forcedist_closedform, Agahi09tcasme_redundancyresolution_tension-velocity, Hassan11tro_tension_analysis, Taghirad11tro_redundancyres_3cases, Gouttefarde15TRO_CableControl} but requires good calibration.  Both offline and online approaches towards calibration through system identification and/or parameter estimation have also been made, but often exhibit tradeoffs between complexity and accuracy.  To our knowledge, existing methods which produce highly dynamic, accurate motions require complex calibration algorithms and/or procedures, while those which are simple to calibrate cannot achieve highly dynamic motion.
% We build on these efforts, implementing a simple manual calibration procedure and task-space feedforward controller, but also introduce time-varying control gains computed using an iLQR algorithm which can achieve highly dynamic motion while being forgiving in the few parameters required.

The design constraints for painting graffiti based on real spray painting data will dictate (a) that a CDPR is an ideal choice of hardware platform, and (b) the design of the CDPR.
% A CDPR is used to render the artwork due to the ability of CDPR to easily scale to large work spaces and achieve highly dynamic motion.

\subsection{Design Constraints}
The primary design requirements for a graffiti painting system center around workspace size, maximum spray can velocity, and maximum spray can acceleration.  We seek a platform which can be easily scaled to 20+ meters square or larger, though in this work we only seek a demonstration sized at a few meters.  Based on the analysis of mocap data presented in Section \ref{ssec:mocap_results}, we determined that we require 7 m/s and 50 m/s$^2$ of speed and acceleration, respectively.  Assuming the mass of the spray can and requisite actuating accessories do not exceed 2kg and compensating for gravity, this means the robot should be capable of exerting 120N upward and 80N downward on the spray can.

Secondary design requirements include portability, extensibility, accuracy, and stiffness.  Portability is central to the goal of producing graffiti artwork in its intended settings outside of a laboratory or studio.  It should be feasible to deconstruct and reconstruct the robot on-site at the wall of a building.  Extensibility of both the workspace and degrees of freedom is desirable to accommodate different artistic visions.  Although the CDPR proposed in this work is planar, adding additional winches to enable 6DoF motion requires relatively little modification.  Finally, accuracy and stiffness are considered secondary constraints because, compared to art forms such as brush painting or sculpture, graffiti is less sensitive to positional inaccuracies and experiences less reaction force.
Based on the thickness of a line painted with a ``needle'' nozzle 5cm from the painting surface, we estimate 2.5cm of repeatability to be sufficient.  We estimate an accuracy of 1\% the size of the painting to be sufficient, based loosely on \cite{Valle56psychol_perceptualThresholds}.
Based on negligible spray paint reaction force and typical wind speeds in Atlanta of 4.1m/s, we estimate external disturbances to be less than 3.1N assuming stagnation pressure applied to a 0.3m$^2$ end-effector.

CDPR present ideal platforms for graffiti painting given the aforementioned requirements.  A CDPR is a robot whose end-effector is pulled by a (redundant) set of cables which are driven by winches on a fixed base.  Thanks to properties of cables, CDPRs can scale to extraordinary sizes and speeds \cite{Nan11ijmp_FAST_telescope, Saptarshi20nasa_lunartelescope}, with the limitation of reduced stiffness to external wrenches.  These qualities make them ideally suited to the large but relatively undisturbed setting and modest accuracy requirement of graffiti painting.

CDPR also have an active research community which has solved many challenges facing CDPRs.  Extensive studies in the late 2000's of CDPR workspace analysis \cite{Bosscher06TRO_wrenchFeasible, Bouchard09_WFW, Gouttefarde11TRO_cableWFW} allow designing CDPR with appropriate workspaces.  Meanwhile, developments in CDPR control and estimation allow real-time control of CDPR, which will be further discussed in Subsection \ref{ssec:cdprControl}.  Preliminarily, based on \cite{Gouttefarde15TRO_CableControl}, we estimate a 1kHz update frequency to be necessary for real-time control.

\subsection{Cable Robot Overview}
% Our CDPR consists of 4 pairs of cables in a planar configuration that can exert pulling forces on the spray can carriage via 4 motor-driven winches.  Each cable pair is driven by the same winch such that their lengths are always matched.  Configuring the cables in pairs provides out-of-plane stabilization with only 4 winches.  The cable mounting positions on the carriage and routing pulley locations are given in Table \ref{tab:cdpr_mountconfig}.
Our CDPR consists of 4 cables in a planar configuration that can exert pulling forces on the end effector (which carries the spray can) via 4 motor-driven winches.  The cable mounting positions on the carriage and routing pulley locations are given in Table \ref{tab:cdpr_mountconfig}.

The frame is constructed from standard 12 gauge steel strut channel to dimensions 3.05m x 2.44m x 0.61m.  The four winches are 2.54cm in diameter with 1.5mm pitch helical grooves to drive 1mm Dyneema® (ultra-high molecular weight polyethylene) rope.  They are driven by 150kV D6374 motors from ODrive Robotics and controlled by two ODrive v3.6 56V motor drives.  The motor drives are connected via separate, isolated CANbuses to a Teensy 4.0 microcontroller (MCU) running at 600MHz which runs the primary CDPR control, sending torque commands and receiving angular position and velocity feedback to/from the motor drives.  The MCU also sends binary spray commands to the spray can actuator wirelessly with an HC-05 bluetooth module.  The MCU is programmed with the closed-loop controller described in Section \ref{ssec:cdprControl}.

The end effector was built from laser cut 5mm hardwood to carry the spray can and actuating electronics.  It consists of the six faces of a box plus two perpendicular midplanes parallel to the gravity vector to center the spray can.  The 4 cables are mounted onto the midplane parallel to the painting surface via 1/4''-20 bolts.

The spray can nozzle actuating mechanism is battery-powered and implemented using a ``20kg'' servo with the lever-arm mechanism from \cite{Liekens20thingiverse_3dprint_spraymount}.  For a full can of Montana BLACK 400mL, the force required to depress the nozzle at the start and end of the stroke was measured to be 20N and 27N, respectively.  The displacement was measured to be 2mm.  Other 400mL spray cans by the brands Montana, Hardcore, and Kobra were used and found to have similar actuation forces and displacements.

\begin{table}
    \centering
    \caption{CDPR cable configuration}
    \begin{tabular}{c|cc}
        \thead{Cable\\ Index} & \thead{End-effector Mounting\\ Location (m)} & \thead{Routing Pulley \\Location (m)}\\
        \hline
        1 & [0.094, -0.061, 0] & [1.52, -1.22, 0] \\
        2 & [0.094, 0.061, 0] & [1.52, 1.22, 0] \\
        3 & [-0.094, 0.061, 0] & [-1.52, 1.22, 0] \\
        4 & [-0.094, -0.061, 0] & [-1.52, -1.22, 0]
    \end{tabular}
    \label{tab:cdpr_mountconfig}
\end{table}

\subsection{Results}
The resulting robot is pictured in Figure \ref{fig:can_actuator}.  The motors are theoretically capable of 600 rad/s and 3.86Nm, which corresponds to 7.62m/s and 94.5m/s$^2$ for the 2.54cm diameter winch, the 1.96e-4 kgm$^2$ motor inertia, and a liberal 2kg end-effector mass.  Thus the designed motor and winch configuration satisfies our design requirements.  The communication via CANbus between the MCU and motor drives was measured to have a feedback-command round-trip latency of 626$\mu$s and easily achieves the required 1kHz update frequency.

The end-effector is pictured in Figure \ref{fig:can_actuator}.  The mass of the empty end-effector was measured to be XXXg, the battery for the nozzle actuator was XXXg, the remaining nozzle actuator components totalled XXXg, and the spray can varied from XXXg to XXXg depending on the fullness and brand.  Thus the total mass varied between XXXg and XXXg.

The spray can actuating mechanism is pictured in Figure \ref{fig:can_actuator} and was able to successfully depress the spray nozzle 100\% of the time in a trial of 100, 1 second long actuations.  The delay between the command to actuate the nozzle and the dispensing of paint was measured to be 400ms.

\begin{figure}
    \centering
    \includegraphics[width=.45\linewidth]{figs/cablerobot.JPG}\\
    \includegraphics[width=.45\linewidth]{figs/paint_actuator.JPG}
    \includegraphics[width=.45\linewidth]{figs/carriage.jpg}
    \caption{Cable robot winch assemblies (top) each consist of a motor controller (shared), motor, and helical winch.  Spray paint actuator (left) uses a servo to depress the spray can nozzle \todo{Gerry}{Update this image with new actuator mechanism}.  End effector (right) carries the spray paint and actuator electronics \todo{Gerry}{replace this potato of an image with a nice one}.}
    \label{fig:can_actuator}
\end{figure}


==> old_09-06/3_software.tex <==
% \subsection{Approach}

From a high-level artistic description in the form of outlines, we need to be able to control the robot to paint graffiti.  We use a hierarchical approach with three levels:

\begin{enumerate}
    \item Path Generation: artistic interpretation and composition of shape placement, overlap, and infill
    % \item ?: closed path determination
    % \item Composition: outline $\rightarrow$ infill $\rightarrow$ outline
    \item Trajectory Generation: interpolation at regular timestamps
    % \item Infill: coverage
    \item CDPR Control: tracking of the desired trajectory
\end{enumerate}

After describing each level, we will quantitatively evaluate the CDPR control and qualitatively evaluate the overall pipeline.

\subsection{Approach: Path Generation} \label{ssec:composition}
\input{3_1_path.tex}

\subsection{Approach: Trajectory Generation}
\input{3_2_traj.tex}

\subsection{Approach: CDPR Control} \label{ssec:cdprControl}
\input{3_3_control.tex}



% The force is converted to cable tensions using a tension distribution (TD) algorithm which seeks to find the minimum tensions needed to achieve the desired force while respecting minimum and maximum cable tension constraints.  Cable tensions and lengths are converted to motor torques and angles by appropriate multiplications with the winch radius and sent to/received from the motor drives.  Forward kinematics (FK) is used to convert cable lengths to the task space pose.

% Loosely based on \cite{Gouttefarde15TRO_CableControl,Lamaury13ICRA_CableControlFF}'s dual-space FF controller, but turns out it's very similar to \cite{Taghirad11tro_redundancyres_3cases} (Fig 3).

% \begin{center}
%     \includegraphics[width=0.4\linewidth]{figs/Taghirad_Fig3.png}
% \end{center}

% \subsubsection{Tension Distribution}
% TD is non-negligible because cable tensions must .... *explain TD*

% \cite{Miermeister16iros_CableRobotSimulator, Pott09ckin_forcedist_closedform} use a closed-form solution which isn't guaranteed to find a solution that exists, but is simple and fast:
% \begin{align}
%     t = t_m - A^{+T}(f+A^Tt_m)
% \end{align}
% where $t_m = (t_{min}+t_{max})/2$ is the ``mean'' feasible tension.
% Note: this is essentially amounts to:
% \begin{align}
%     t = (I-A^{T+}A^T)t_m -A^{T+}f
% \end{align}
% which essentially amounts to a special case of \cite{Agahi09tcasme_redundancyresolution_tension-velocity} which just specifies to find an "optimal" feasible solution to the problem:
% \begin{align}
%     t = t_p + (I-A^{T+}A^T)\lambda
% \end{align}
% For the case of $n+1$ cables, $\lambda$ is a scalar and has $n+1$ inequalities to satisfy.

% \cite{Hassan11tro_tension_analysis} uses an iterative approach based on Dykstra's alg: project $t$ onto the space that satisfies wrench balance, then project onto space that satisfies tension inequalities and repeat until convergence.  Not-deterministic, obviously.  Another interesting quote: ``Although higher cable tensions are desirable be- cause they result in higher stiffness [31], they require bigger motors and lead to a greater operating cost. In addition, higher tensions lead to excessive cable elongation, generating greater positioning error at the end effector.''

% \cite{Taghirad11tro_redundancyres_3cases} uses KKT to solve the LP and explicitly lays out 3 cases for the inequality constraints: none active, some active, all active.  For the ``some active'' case, solve the equality case for the active constraints for every possible combination of active constraints and check if it's feasible.

% \cite{Lamaury13ICRA_CableControlFF, Gouttefarde15TRO_CableControl} are basically the same as each-other and give an efficient algorithm for tension distribution for the $n+2$ cables case based on linear programming.  Start with a (possibly infeasible) point with 2 inequalities active.  One stays active and the other becomes inactive, then follow until hitting the next inequality constraint.  Repeat until form a loop -- the loop defines the feasible polygon in 2-D ``free parameter space''.  Use whatever algorithm (i.e. centroid) to find optimal distribution within 2D feasible polygon.

% We choose to use a slight modification of the version proposed by \cite{Pott09ckin_forcedist_closedform}:
% \begin{align}
%     t = t_{min} + M2(f+A^Tt_{min})
% \end{align}
% where M2 is a hard-coded solution to the LP problem that enumerates all 4 cases where 2/4 adjacent inequality constraints are active.

\subsubsection{State Estimation} \label{sec:software_estimation}
Although FK for CDPR typically uses a nonlinear least squares solver to estimate position, we found that naively discarding redundant information is sufficient for our graffiti application.  Since CDPR are over-actuated, *explain FK*.  Instead, we simply apply geometry using the top two cable lengths to estimate the spray can position, and we assume the spray can is always vertical.  We find that this is typically a safe assumption for our application with quantitative results discussed in Section \ref{ssec:software_results}.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/blockdiagram_4tension.png}
    \caption{OUT OF DATE!!!!!!!  Ignore the ``TD'' block, and the Ki/Kp/Kd gains come from GTSAM. %Cable robot controller applies PID control in the task space to obtain force which is converted to cable tensions with a tension distribution (TD) block.  Forward kinematics (FK) converts cable lengths back to task space.
    }
    \label{fig:blockdiagram}
\end{figure}



==> old_09-06/4_record.tex <==
We first capture artwork using an OptiTrack™ mocap system for its simplicity and accuracy.  Mocap systems have the advantage of directly outputting positions and orientations of rigid bodies with sub-millimeter accuracy which trivializes the process of obtaining the 6D trajectories of a spray paint can during painting.  Although motion capture systems significantly hinder the accessibility and mobility of capture systems, we argue that they present an excellent first step in outlining how graffiti preservation can be improved through real-world recreations.  We also note that, as we will discuss in Section \ref{sec:software}, the processing and rendering components of our pipeline can also use other forms of captured artwork such as svg and GML files in addition to mocap data.

We collect a library of simple shapes which can later be composed.
% In this work, we collect each letter of the English alphabet along with a few simple line drawings for each of our two artist collaborators.
Additional tags, characters, and full murals can be added to the library in the future.

\subsection{Methods}
\subsubsection{Data Collection Procedure}
We collected the full 6D trajectories of the spray cans and painting surfaces (plywood sheets) as two graffiti artist collaborators painted various symbols.  The spray can positions and orientations were obtained by affixing 4 mocap position markers to fixed positions relative to the cans via a 3D printed structure as shown in Figure \ref{fig:capture_spraycan}.  Similarly, the markers were placed on the 4 corners of the painting surface.  From the 4 position tracks, OptiTrack's Motive™ software was able to automatically extract the 6DoF poses of the cans and plywood for each time step at 120Hz.  One additional marker was placed on the tip of the artist's index finger to aid in identifying when the spray can nozzle was depressed.  During data collection, reflective objects were covered in painter's tape to reduce mocap tracking failures.  For each art collaborator, the 26 letters of the English alphabet were captured along with special symbols such as punctuation marks and a small doodle of the artists' choices (skull).

\begin{figure}
    \centering
    \includegraphics[width=.5\linewidth]{figs/mocap_paintcan.jpg}
    \caption{4 mocap position markers (gray) affixed to a spray paint can via 3D printed structure (white) to track 6DoF spray can pose.}
    \label{fig:capture_spraycan}
\end{figure}

\subsubsection{Data Pre-processing}
The motion capture data is given in arbitrary ``world'' coordinates so we must convert the data into the painting surface's reference frame.
% We apply coordinate transformations to obtain the spray can trajectory relative to the painting surface.  
The top left (y-axis), bottom left (origin), and bottom right (x-axis) markers of the painting surface are used to obtain the coordinate frame, ${}_wT_s[k]$, of the \underline{s}urface in the \underline{w}orld frame for each timestep, $k$, using Gram-Schmidt Orthogonalization for x then y, then using the cross product to obtain the z-axis.  Anecdotally, we found that the fourth mocap marker was never needed, though it would be useful in the event of one of the other three markers missing data.  For the spray can, a similar process is performed to obtain the \underline{c}an's frame, ${}_wT_c[k]$.  The pose of the spray can's \underline{n}ozzle in the spray can's frame, ${}_cT_n$, is obtained by manually measuring the position in the spray can's coordinate system and assigning the identity rotation.  Finally, the nozzle's pose in the painting surface's frame at timestep $k$, ${}_s^kT_n$, can be expressed as
\begin{align*}
    {}_sT_n[k] &= ({}_wT_s^{-1}[k]) ~({}_wT_c[k]) ~ (_cT_n)
\end{align*}

To determine when the spray nozzle is being depressed (painting vs traveling motions), we compute the position of the finger marker in the can's frame and apply a threshold y-value.  We then manually review and repair any incorrect classifications.

\subsubsection{Informing Robot Hardware Requirements}
As an additional analysis, we also study the speeds and accelerations reached by our collaborating artists during painting and traveling to inform the necessary capabilities of the cable robot hardware.

\subsection{Results} \label{ssec:mocap_results}
We believe the data we collected of artists as they were painting is one of the most realistic and accurate descriptions of graffiti art in the literature to allow human-robot artistic collaboration.  The resulting 6DoF trajectories of the spray nozzle and its depressed vs un-depressed states are sufficient for the rest of our system to recreate the original artwork.
Figure \ref{fig:mocap_max} shows an example of the mocap data projected onto the painting surface, with painting vs traveling denoted as blue and red respectively.

\begin{figure} % h! is placeholder
    \centering
    \includesvg[width=.5\linewidth]{figs/Max-name.svg}
    \caption{Plot of painting motion of the name "Max" from motion capture data}
    \label{fig:mocap_max}
\end{figure}

The speeds and accelerations reached by the human graffiti artists is shown in Figure \ref{fig:mocap_histograms}.  We decided to set the minimum cable robot hardware requirements to 7m/s and 50m/s$^2$ of acceleration.

\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{figs/mocapSpeedAcc_Max.png}
    \caption{Speeds and accelerations typical of a human graffiti artist which define design constraints of the cable robot}
    \label{fig:mocap_histograms}
\end{figure}



==> old_09-06/5_results_discussion.tex <==
% Possible other quantitative experiments:
%     Image accuracy?
%     Experiment: capture robot painting w/ mocap and re-create robot painting with full pipeline; see how well they match.

\begin{figure}
    \centering
    \includegraphics[width=.75\linewidth]{figs/iros_logo_3_track_traj3.png}
    \caption{Setpoint, estimated, and ground truth trajectories of the ``IROS'' logo as executed by the cable robot graffiti painting system.}
    \label{fig:iros_logo_traj}
\end{figure}

\subsubsection{Estimation Accuracy}
To evaluate the accuracy of the position estimation (forward kinematics) procedure described in Section \ref{sec:software_estimation}, the ground truth positions were measured using the same mocap hardware used to capture the graffiti art, and the estimated positions were logged at 100Hz while executing the same trajectory that generated Figure \ref{fig:iros_logo_traj}.  The mocap coordinates were aligned to x/y cable robot coordinates from the 4 corner pulley locations.  To align the discrete samples from the 60Hz mocap data and 100Hz robot log, the robot log data was piecewise linearly interpolated.

The results, shown in Figure \ref{fig:iros_logo_estimation}, show that the spray can position estimate using the procedure described in Section \ref{sec:software_estimation} is sufficiently accurate for graffiti painting, with an average position error of 19mm $\pm$ 10mm.

\begin{figure}
    \centering
    \includegraphics[width=.75\linewidth]{figs/iros_logo_3_track_estimation.png}
    \caption{Ground truth and online estimate of spray can x/y position (top) and error (bottom).  The resolution of the ground truth is 10mm}
    \label{fig:iros_logo_estimation}
\end{figure}

\subsubsection{Controller Tracking Ability}
We tested 3 different controllers to determine that the iLQR-based controller was the most suitable for our graffiti painting application.

To evaluate the ability of the controllers to track graffiti trajectories, the setpoint and estimated positions of the spray can were logged while executing three test trajectories: (1) the same trajectory that generated Figure \ref{fig:iros_logo_traj}, (2) a step input, and (3) a set of concentric rectangles.

% The results, shown in Figure \ref{fig:iros_logo_control}, show that slow-speed tracking is very accurate while tracking at higher speeds is limited by the controller's bandwidth.  Lower latency, which enables higher gains without sacrificing phase margin, and a feed-forward controller \cite{Lamaury13ICRA_CableControlFF, Gouttefarde15TRO_CableControl} are expected to improve high-speed tracking performance.

The results, shown in Figure ???, show that our controller is better.  A PARAGRAPH OF DISCUSSION GOES HERE.

\begin{figure}
    \centering
    \includegraphics[width=.75\linewidth]{figs/iros_logo_3_track_control.png}
    \caption{Setpoint and estimated positions of the spray can x/y position indicate approximately 400ms of delay between \todo{gerry}{Describe in terms of bandwidth, and maybe use step functions instead of arbitrary trajectory}}
    \label{fig:iros_logo_control}
\end{figure}

\subsubsection{Graffiti Art}
We present qualitative results of our graffiti art, including ``ATL'' (for Atlanta), ``GTSAM'', and the logo for ICRA 2022 alongside their reference inputs.  in Figure \ref{fig:iros_logo_3_img}.  \todo{Gerry}{this section}

\begin{figure}
    \centering
    \includegraphics[width=.75\linewidth]{figs/iros_logo_3_img.jpg}
    \caption{A completed graffiti painting of the ``IROS'' logo \todo{Gerry}{put real photo here, of the mocap version of some word}}
    \label{fig:iros_logo_3_img}
\end{figure}

